Efficient & Correct Predictive Equivalence for Decision Trees

The Rashomon set of decision trees (DTs) finds importance uses. Recent work showed that DTs computing the same classification function, i.e. predictive equivalent DTs, can represent a significant fraction of the Rashomon set. Such redundancy is undesirable. For example, feature importance based on the Rashomon set becomes inaccurate due the existence of predictive equivalent DTs, i.e. DTs with the same prediction for every possible input. In recent work, McTavish et al. proposed solutions for several computational problems related with DTs, including that of deciding predictive equivalent DTs. The approach of McTavish et al. consists of applying the well-known method of Quine-McCluskey (QM) for obtaining minimum-size DNF (disjunctive normal form) representations of DTs, which are then used for comparing DTs for predictive equivalence. Furthermore, the minimum-size DNF representation was also applied to computing explanations for the predictions made by DTs, and to finding predictions in the presence of missing data. However, the problem of formula minimization is hard for the second level of the polynomial hierarchy, and the QM method may exhibit worst-case exponential running time and space. This paper first demonstrates that there exist decision trees that trigger the worst-case exponential running time and space of the QM method. Second, the paper shows that the QM method may incorrectly decide predictive equivalence, if two key constraints are not respected, and one may be difficult to formally guarantee. Third, the paper shows that any of the problems to which the smallest DNF representation has been applied to can be solved in polynomial time, in the size of the DT. The experiments confirm that, for DTs for which the worst-case of the QM method is triggered, the algorithms proposed in this paper are orders of magnitude faster than the ones proposed by McTavish et al.

==> algs/truepathbool.tex <==
\begin{flushleft}
  \hspace*{\algorithmicindent}
  \textbf{Input}: {$\fml{A}$: partial assignment; $P$: path; $\fml{T}$: DT}\\
  \hspace*{\algorithmicindent}
  \textbf{Output}: {$\top$ if path $P$ consistent with $\mbf{x}$;
    else $\bot$}\\
\end{flushleft}

\begin{algorithmic}[1]
  \Function{$\truepath$}{$\fml{A}$, $P$, $\fml{T}$}
  \State{$s_b\gets\isterm(P; \fml{T})$}
  \State{$s_a\gets\pnode(s_b; \fml{T})$}
  \While{$s_a\not=\msf{none}$}
  \If{$\neg\holds(\fml{A}, \elit(s_a,s_b;\fml{T}))$}
  \State{\Return $\bot$}
  \EndIf
  \State{$(s_a,s_b)\gets(\pnode(s_a; \fml{T}), s_a)$}
  \EndWhile
  \State{\Return $\top$}
  \EndFunction
\end{algorithmic}


==> texfigs/km01.tex <==
\begin{comment}
%
\begin{Karnaugheight}
  \minterms{0,4,5,10,11,13,15}
  \maxterms{1,2,3,6,7,8,9,12,14}
  %\implicantcostats{0}{2}{green}
  \implicantsol{7}{green}
  %\implicant{0}{1}{green}
  \implicant{0}{4}{green}
  \implicant{4}{5}{green}
  \implicant{5}{13}{green}
  \implicant{13}{15}{green}
  \implicant{15}{11}{green}
  \implicant{11}{10}{green}
  %%\implicant{10}{0}{green}
\end{Karnaugheight}
%
\end{comment}
%
\begin{karnaugh-map}[4][4][1][$x_2x_1$][$x_4x_3$]
  \minterms{0,1,5,7,8,10,14,15}
  \implicant{0}{1}
  \implicant{1}{5}
  \implicant{5}{7}
  \implicant{7}{15}
  \implicant{15}{14}
  \implicant{14}{10}
  \implicantedge{8}{8}{10}{10}
  \implicantedge{0}{0}{8}{8}
  \autoterms[0]
\end{karnaugh-map}


==> texfigs/twogadgets.tex <==
\tikzset{>=Stealth}
\begin{tikzpicture}[->,%
  ]
  \node[] (1) at (0,0) {\input{./texfigs/gadget1}};
  \node[] (2) at (3.385,-1.0) {\input{./texfigs/gadget2}};
  \node[] (3) at (-1.5,-3.0) {(a) Main gadget};
  \node[] (4) at (3.35,-3.0) {(b) Last gadget};
  %
\end{tikzpicture} 


==> wip.tex <==
\section{Introduction}

\blindmathpaper

Here is a citation \cite{chow:68}.

% Acknowledgements and Disclosure of Funding should go at the end, before appendices and references

\acks{All acknowledgements go at the end of the paper before appendices and references.
Moreover, you are required to declare funding (financial activities supporting the
submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found on the JMLR website.}

% Manual newpage inserted to improve layout of sample file - not
% needed in general before appendices/bibliography.

\newpage

\appendix
\section{}
\label{app:theorem}

% Note: in this sample, the section number is hard-coded in. Following
% proper LaTeX conventions, it should properly be coded as a reference:

%In this appendix we prove the following theorem from
%Section~\ref{sec:textree-generalization}:

In this appendix we prove the following theorem from
Section~6.2:

\noindent
{\bf Theorem} {\it Let $u,v,w$ be discrete variables such that $v, w$ do
not co-occur with $u$ (i.e., $u\neq0\;\Rightarrow \;v=w=0$ in a given
dataset $\dataset$). Let $N_{v0},N_{w0}$ be the number of data points for
which $v=0, w=0$ respectively, and let $I_{uv},I_{uw}$ be the
respective empirical mutual information values based on the sample
$\dataset$. Then
\[
	N_{v0} \;>\; N_{w0}\;\;\Rightarrow\;\;I_{uv} \;\leq\;I_{uw}
\]
with equality only if $u$ is identically 0.} \hfill\BlackBox

\section{}

\noindent
{\bf Proof}. We use the notation:
\[
P_v(i) \;=\;\frac{N_v^i}{N},\;\;\;i \neq 0;\;\;\;
P_{v0}\;\equiv\;P_v(0)\; = \;1 - \sum_{i\neq 0}P_v(i).
\]
These values represent the (empirical) probabilities of $v$
taking value $i\neq 0$ and 0 respectively.  Entropies will be denoted
by $H$. We aim to show that $\fracpartial{I_{uv}}{P_{v0}} < 0$....\\

{\noindent \em Remainder omitted in this sample. See http://www.jmlr.org/papers/ for full paper.}

